Overcoming the Price of Anarchy by Steering with Recommendations

Varied real world systems such as transportation networks, supply chains and energy grids present coordination problems where many agents must learn to share resources. It is well known that the independent and selfish interactions of agents in these systems may lead to inefficiencies, often referred to as the `Price of Anarchy'. Effective interventions that reduce the Price of Anarchy while preserving individual autonomy are of great interest. In this paper we explore recommender systems as one such intervention mechanism. We start with the Braess Paradox, a congestion game model of a routing problem related to traffic on roads, packets on the internet, and electricity on power grids. Following recent literature, we model the interactions of agents as a repeated game between $Q$-learners, a common type of reinforcement learning agents. This work introduces the Learning Dynamic Manipulation Problem, where an external recommender system can strategically trigger behavior by picking the states observed by $Q$-learners during learning. Our computational contribution demonstrates that appropriately chosen recommendations can robustly steer the system towards convergence to the social optimum, even for many players. Our theoretical and empirical results highlight that increases in the recommendation space can increase the steering potential of a recommender system, which should be considered in the design of recommender systems.

==> bios/bios.tex <==
{Cesare Carissimo}
Cesare Carissimo is pursuing a Ph.D. at ETH Zürich with a focus on machine behaviour, complex systems, economics and game theory. He has an interdisciplinary background with a B.S. from the Faculty of Politics, Psychology, Law and Economics, and a M.S. of Computational Science from the University of
Amsterdam.

(Marcin Korecki)
Marcin Korecki is a researcher specializing in artificial intelligence, complexity, and philosophy. He earned his PhD from ETH Zurich, focusing on interdisciplinary work in these areas. His academic experience includes studies at the University of Groningen in the Netherlands and the University of Edinburgh in Scotland. During his PhD, he also spent six months at the University of Tokyo in Japan.

{Damian Dailisan }
is currently a postdoctoral researcher at ETH Z\"urich. He obtained his B.S. in applied physics in 2015 and his M.S. (2017) and Ph.D. (2020) degrees in physics from the University of the Philippines Diliman. After obtaining his Ph.D., he worked as a Data Scientist and Adjunct Professor at the Asian Institute of Management (2021). His research interests include phase transitions in agent-based cellular automata traffic models, data science, reinforcement learning, and AI.
